How Important Is a Neuron?

The problem of attributing a deep network's prediction to its \emph{input/base} features is well-studied. We introduce the notion of \emph{conductance} to extend the notion of attribution to the understanding the importance of \emph{hidden} units. Informally, the conductance of a hidden unit of a deep network is the \emph{flow} of attribution via this hidden unit. We use conductance to understand the importance of a hidden unit to the prediction for a specific input, or over a set of inputs. We evaluate the effectiveness of conductance in multiple ways, including theoretical properties, ablation studies, and a feature selection task. The empirical evaluations are done using the Inception network over ImageNet data, and a sentiment analysis network over reviews. In both cases, we demonstrate the effectiveness of conductance in identifying interesting insights about the internal workings of these networks.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

We propose a notion of conductance that extends the notion of attribution to capture the importance of a hidden unit (neuron, or a group of related neurons).
Conductance both identifies the importance of the hidden unit, and explains its function.
We demonstrate the versatility of the method by applying it to a deep network that works with  images, and another that operates on text.
The method is easy to apply. It does not require the network to be instrumented and can be applied with a few lines of code in your favorite machine-learning framework.

In this paper, we analyzed groups of (logically related) neurons. How do we
select such groups to analyze? While most networks at first glance may seem
like monolithic black-boxes,
the networks do implicitly employ abstractions. In the networks we analyzed, the abstraction was that of a filter.
All networks implicitly have abstractions, for instance, the notion of attention neurons in sequence to sequence networks.
The quality of the analysis does depend on a careful choice of what group of neurons to analyze.
Though it is not clear how to automate this, designers of networks typically have good intuition
for their choice of abstractions, and they often describe this in papers, which may guide the choice of what to analyze.

The ability to perform analysis at levels higher levels of abstraction than a base feature (pixel/word) also helps with sanity checking.
Attributions and conductance are implicitly causal claims about the importance of features. It is natural to verify these claims with ablations.
Ablations at the level of base features are often ineffective as we discussed in Section~\ref{sec:contribution}.
Consequently, most of the attribution literature does not have an empirical sanity check.
In contrast, we show that the conductances of hidden units at the right level of abstraction do agree with ablation scores, which is a useful sanity check.

Finally, why study conductances? The literature on understanding behavior of
hidden units is typically motivated by the increase in trust on deep networks
that stems from interpretability (cf.~\cite{featurevis}).
We agree with this motivation. Furthermore, conductances raise the level of the
explanation to higher-level features, which could help with interpretability.
For instance, it may be possible to label every filter in the Inception network
from Section~\ref{sec:object} by hand; for instance Filter $52$ in $mixed3a$ as
``glare'' (cf. Figure~\ref{fig:collisions} and so on. This could be used to
produce a natural language explanation: ``Half of the network's prediction was
because of shape, and about $20\%$ was because of the glare...''
Additionally, it is possible that conductance is useful as an analytical aid in
improving networks. In the sentiment model (Section~\ref{sec:sentiment}), there
are filters of four widths that range from $3$ words to $6$ words.
There are $64$ filters for each width. But we find that the $30\%$ of the
conductance magnitude flows through the filter of the largest size. Perhaps one
could increase the number of filters at this size? Or add filters with higher
widths? Designers of networks often have intuition for why they added certain
module to the network. Conductances could help quantitatively verify such
intuition. A different application of conductance is indicated by
Figures~\ref{fig:not-good} and~\ref{fig:not-bad}. Perhaps conductance could
help harvest rules for use in a rule-based system. Unlike image models,
optimization based techniques like DeepDream~\cite{deepdream} have not been
shown to work effectively for text-based models. The approach in
Section~\ref{sec:negation} seems fairly general: Identify hidden units high
conductance for an exemplar of the rule, and then run a large number of
examples through the network, extracting phrases that have a high conductance
for these high-conductance units.

